Translating Under Pressure: Domain-Aware LLMs for Crisis Communication

Timely and reliable multilingual communication is critical during natural and human-induced disasters, but developing effective solutions for crisis communication is limited by the scarcity of curated parallel data. We propose a domain-adaptive pipeline that expands a small reference corpus, by retrieving and filtering data from general corpora. We use the resulting dataset to fine-tune a small language model for crisis-domain translation and then apply preference optimization to bias outputs toward CEFR A2-level English. Automatic and human evaluation shows that this approach improves readability, while maintaining strong adequacy. Our results indicate that simplified English, combined with domain adaptation, can function as a practical lingua franca for emergency communication when full multilingual coverage is not feasible.

==> scatter_plot.tex <==
\begin{figure}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}
\begin{axis}[
    width=10cm,
    height=7cm,
    scale only axis,
    xlabel={Weighted MQM score},
    ylabel={DA score},
    xmin=-25, xmax=0,
    ymin=0, ymax=105,
    x dir=reverse,
    xtick={0,-5,-10,-15,-20,-25},
    grid=major,
    grid style={dashed,gray!30},
    axis lines=left,
]
\path[fill=blue!8, draw=none]
    (axis cs:-25,70) rectangle (axis cs:0,105);

\addplot[
    scatter,
    only marks,
    scatter src=explicit,
    mark=*,
    opacity=0.6,
    visualization depends on=\thisrow{count} \as \size,
    scatter/@pre marker code/.code={
        \pgfplotsset{mark size={sqrt(\size)}}
    },
] table {
x y count
0 100 81
-1 90 27
-2 80 11
-3 70 7
-5 80 6
-2 70 6
-3 60 5
-5 65 5
-6 55 4
-7 45 3
-10 45 2
-12 35 2
-6 50 2
-1 80 8
-1 75 3
-2 75 3
-5 70 4
-2 85 2
-1 85 2
-7 60 3
-4 60 3
-6 70 4
-2 60 2
-5 60 2
-11 30 1
-12 25 1
-11 20 1
-22 20 1
};

\end{axis}
\end{tikzpicture}
}
\caption{Relationship between weighted MQM and DA scores for the DPO model.}
\end{figure}

